Variability of wave power production of the M4 machine at two energetic open ocean locations: off Albany, Western Australia and at EMEC, Orkney, UK

Since intermittent and highly variable power supply is undesirable, quantifying power yield fluctuations of wave energy converters (WECs) aids with assessment of potential deployment sites. This paper presents analysis of 3-hourly, monthly, seasonal, and inter-annual variability of power output of the M4 WEC. We compare expected performance from deployment at two wave energy hotspots: off Albany on the south-western coast of Australia and off the European Marine Energy Centre (EMEC) at Orkney, UK. We use multi-decadal wave hindcast data to predict the power that would have been generated by M4 WEC machines. The M4 machine, as a floating articulated device which extracts energy from flexing motion about a hinge, is sized according to a characteristic wavelength of the local wave climate. Using probability distributions, production duration curves, and coefficients of variation we demonstrate larger variability of the 3-hourly power yield at Orkney compared to Albany. At longer timescales, seasonal trends are highlighted through average monthly power values. From a continuity of supply perspective, we investigate occurrences of low production at three different threshold levels and calculate duration and likelihood of such events. Orkney is found to suffer from more persistent lows, causing a more intermittent power output. We also consider the effect of machine size on its power performance. Smaller machines are found to more effectively smooth out the stochastic nature of the underlying wave resource.

==> extra_refs_from_Harrif_orig_doc.tex <==



@article{santo2017extreme,
  title={Extreme motion and response statistics for survival of the three-float wave energy converter M4 in intermediate water depth},
  author={Santo, H and Taylor, PH and Carpintero Moreno, E and Stansby, P and Taylor, R Eatock and Sun, L and Zang, J},
  journal={Journal of Fluid Mechanics},
  volume={813},
  pages={175--204},
  year={2017},
  publisher={Cambridge University Press}
}



@article{bidlot2016,
  title={{Hindcast hourly data from ECWAM (CY41R1) using ERA-Interim forcing from 1979 to 2014}},
  author={Bidlot, J},
  journal={Private communication},
  year={2016},
  publisher={Wiley Online Library}
}



@article{reguero2015global,
  title={A global wave power resource and its seasonal, interannual and long-term variability},
  author={Reguero, BG and Losada, IJ and M{\'e}ndez, FJ},
  journal={Applied Energy},
  volume={148},
  pages={366--380},
  year={2015},
  publisher={Elsevier}
}

@article{stansby2015capture,
  title={{Capture width of the three-float multi-mode multi-resonance broadband wave energy line absorber M4 from laboratory studies with irregular waves of different spectral shape and directional spread}},
  author={Stansby, Peter and Moreno, Efrain Carpintero and Stallard, Tim},
  journal={Journal of Ocean Engineering and Marine Energy},
  pages={1--12},
  year={2015},
  publisher={Springer}
}

@article{stansby2015three,
  title={Three-float broad-band resonant line absorber with surge for wave energy conversion},
  author={Stansby, P and Moreno, E Carpintero and Stallard, T and Maggi, A},
  journal={Renewable Energy},
  volume={78},
  pages={132--140},
  year={2015},
  publisher={Elsevier}
}

@article{eatocktaylor2015coupled,
  title={{A coupled hydrodynamic-structural model of the M4 wave energy converter}},
  author={Eatock Taylor, R. and Taylor, P. H. and Stansby, P. K.},
  journal={Journal of Fluids and Structures (under review)},
  year={2015},
  publisher={Elsevier}
}





@article{vinoth2011global,
  title={Global estimates of extreme wind speed and wave height},
  author={Vinoth, J and Young, IR},
  journal={Journal of Climate},
  volume={24},
  number={6},
  pages={1647--1665},
  year={2011}
}

@article{izaguirre2011global,
  title={Global extreme wave height variability based on satellite data},
  author={Izaguirre, Cristina and M{\'e}ndez, Fernando J and Men{\'e}ndez, Melisa and Losada, Inigo J},
  journal={Geophysical Research Letters},
  volume={38},
  number={10},
  year={2011},
  publisher={Wiley Online Library}
}

@article{izaguirre2010extreme,
  title={{Extreme wave climate variability in southern Europe using satellite data}},
  author={Izaguirre, Cristina and Mendez, Fernando J and Menendez, Melisa and Luce{\~n}o, Alberto and Losada, Inigo J},
  journal={Journal of Geophysical Research: Oceans (1978--2012)},
  volume={115},
  number={C4},
  year={2010},
  publisher={Wiley Online Library}
}

@article{menendez2008variability,
  title={{Variability of extreme wave heights in the northeast Pacific Ocean based on buoy measurements}},
  author={Men{\'e}ndez, Melisa and M{\'e}ndez, Fernando J and Losada, Inigo J and Graham, Nicholas E},
  journal={Geophysical Research Letters},
  volume={35},
  number={22},
  year={2008},
  publisher={Wiley Online Library}
}

@inproceedings{tromans1995response,
  title={{Response based design method in the north sea: Application of a new method}},
  author={Tromans, P and Vanderschuren, L},
  booktitle={Offshore Technology Conference, OTC 7683, Houston},
  year={1995}
}

@inproceedings{taylor2000extrapolation,
  title={{Extrapolation of long-term storm statistics, the POT method and data transformation}},
  author={Taylor, PH and Goh, GYK},
  booktitle={Proceedings of the 19th International Conference on Offshore Mechanics and Arctic Engineering, New Orleans},
  year={2000}
}

@inproceedings{taylor2009100,
  title={100-year waves, teleconnections and wave climate variability},
  author={Taylor, PH and Barker, VE and Bishop, D and Eatock Taylor, R},
  booktitle={17th International Workshop on Wave Hindcasting and Forecasting, Halifax, Canada},
  year={2009}
}

@article{wang2001changes,
  title={{Changes of extreme wave heights in Northern Hemisphere oceans and related atmospheric circulation regimes}},
  author={Wang, Xiaolan L and Swail, Val R},
  journal={Journal of Climate},
  volume={14},
  number={10},
  pages={2204--2221},
  year={2001}
}

@article{caires2005100,
  title={{100-year return value estimates for ocean wind speed and significant wave height from the ERA-40 data}},
  author={Caires, S and Sterl, A},
  journal={Journal of Climate},
  volume={18},
  number={7},
  pages={1032--1048},
  year={2005}
}

@article{wentz2007much,
  title={How much more rain will global warming bring?},
  author={Wentz, Frank J and Ricciardulli, Lucrezia and Hilburn, Kyle and Mears, Carl},
  journal={Science},
  volume={317},
  number={5835},
  pages={233--235},
  year={2007},
  publisher={American Association for the Advancement of Science}
}

@article{young2012investigation,
  title={Investigation of trends in extreme value wave height and wind speed},
  author={Young, IR and Vinoth, J and Zieger, S and Babanin, AV},
  journal={Journal of Geophysical Research: Oceans (1978--2012)},
  volume={117},
  number={C11},
  year={2012},
  publisher={Wiley Online Library}
}

@article{young2011global,
  title={Global trends in wind speed and wave height},
  author={Young, IR and Zieger, S and Babanin, AV},
  journal={Science},
  volume={332},
  number={6028},
  pages={451--455},
  year={2011},
  publisher={American Association for the Advancement of Science}
}

@article{zieger2014changes,
  title={Changes in ocean surface wind with a focus on trends in regional and monthly mean values},
  author={Zieger, S and Babanin, AV and Young, IR},
  journal={Deep Sea Research Part I: Oceanographic Research Papers},
  volume={86},
  pages={56--67},
  year={2014},
  publisher={Elsevier}
}

@article{shimura2013ocean,
  title={Ocean waves and teleconnection patterns in the northern hemisphere},
  author={Shimura, Tomoya and Mori, Nobuhito and Mase, Hajime},
  journal={Journal of Climate},
  volume={26},
  number={21},
  pages={8654--8670},
  year={2013}
}

@article{woollings2010variability,
  title={{Variability of the North Atlantic eddy-driven jet stream}},
  author={Woollings, Tim and Hannachi, Abdel and Hoskins, Brian},
  journal={Quarterly Journal of the Royal Meteorological Society},
  volume={136},
  number={649},
  pages={856--868},
  year={2010},
  publisher={Wiley Online Library}
}

@article{woollings2014contrasting,
  title={{Contrasting interannual and multidecadal NAO variability}},
  author={Woollings, T and Franzke, Christian and Hodson, DLR and Dong, B and Barnes, EA and Raible, CC and Pinto, JG},
  journal={Climate Dynamics},
  pages={1--18},
  year={2014},
  publisher={Springer}
}

@article{smith2014seasonal,
  title={{Seasonal to decadal prediction of the winter North Atlantic Oscillation: emerging capability and future prospects}},
  author={Smith, Doug M and Scaife, Adam A and Eade, Rosie and Knight, Jeff R},
  journal={Quarterly Journal of the Royal Meteorological Society},
  year={2014},
  publisher={Wiley Online Library},
  doi={10.1002/qj.2479}
}

@article{cassou2011statistical,
  title={{A statistical--dynamical scheme for reconstructing ocean forcing in the Atlantic. Part I: weather regimes as predictors for ocean surface variables}},
  author={Cassou, Christophe and Minvielle, Marie and Terray, Laurent and P{\'e}rigaud, Claire},
  journal={Climate Dynamics},
  volume={36},
  number={1-2},
  pages={19--39},
  year={2011},
  publisher={Springer}
}

@article{bacon1991wave,
  title={{Wave climate changes in the North Atlantic and North Sea}},
  author={Bacon, S and Carter, DJT},
  journal={International Journal of Climatology},
  volume={11},
  number={5},
  pages={545--558},
  year={1991},
  publisher={Wiley Online Library}
}

@article{bacon1993connection,
  title={{A connection between mean wave height and atmospheric pressure gradient in the North Atlantic}},
  author={Bacon, S and Carter, DJT},
  journal={International Journal of Climatology},
  volume={13},
  number={4},
  pages={423--436},
  year={1993},
  publisher={Wiley Online Library}
}

@article{carter1988has,
  title={{Has the north-east Atlantic become rougher?}},
  author={Carter, DJT and Draper, L},
  journal={Nature},
  volume={332},
  pages={494},
  year={1988}
}

@article{allan2000ocean,
  title={{Are ocean wave heights increasing in the eastern North Pacific?}},
  author={Allan, Jonathan and Komar, Paul},
  journal={EOS, Transactions American Geophysical Union},
  volume={81},
  number={47},
  pages={561--567},
  year={2000},
  publisher={Wiley Online Library}
}

@book{von2001statistical,
  title={Statistical Analysis in Climate Research},
  author={Von Storch, Hans and Zwiers, Francis W},
  year={2001},
  publisher={Cambridge university press}
}

@article{kushnir1997recent,
  title={{The recent increase in North Atlantic wave heights}},
  author={Kushnir, Y and Cardone, VJ and Greenwood, JG and Cane, MA},
  journal={Journal of Climate},
  volume={10},
  number={8},
  pages={2107--2113},
  year={1997}
}

@article{hurrell1995decadal,
  title={{Decadal trends in the North Atlantic Oscillation: regional temperatures and precipitation}},
  author={Hurrell, James W},
  journal={Science},
  volume={269},
  number={5224},
  pages={676--679},
  year={1995},
  publisher={American Association for the Advancement of Science}
}

@article{moore2013multidecadal,
  title={{Multidecadal mobility of the North Atlantic Oscillation}},
  author={Moore, GWK and Renfrew, IA and Pickart, Robert S},
  journal={Journal of Climate},
  volume={26},
  number={8},
  pages={2453--2466},
  year={2013}
}

@article{barnston1987classification,
  title={Classification, seasonality and persistence of low-frequency atmospheric circulation patterns},
  author={Barnston, Anthony G and Livezey, Robert E},
  journal={Monthly Weather Review},
  volume={115},
  number={6},
  pages={1083--1126},
  year={1987}
}

@article{hurrell2010north,
  title={{North Atlantic climate variability: the role of the North Atlantic Oscillation}},
  author={Hurrell, James W and Deser, Clara},
  journal={Journal of Marine Systems},
  volume={79},
  number={3},
  pages={231--244},
  year={2010},
  publisher={Elsevier}
}

@article{uppala2005era,
  title={{The ERA-40 re-analysis}},
  author={Uppala, Sakari M and K{\aa}llberg, PW and Simmons, AJ and Andrae, U and Bechtold, V and Fiorino, M and Gibson, JK and Haseler, J and Hernandez, A and Kelly, GA and others},
  journal={Quarterly Journal of the Royal Meteorological Society},
  volume={131},
  number={612},
  pages={2961--3012},
  year={2005},
  publisher={Wiley Online Library}
}

@article{tsimplis2005towards,
  title={{Towards a vulnerability assessment of the UK and northern European coasts: the role of regional climate variability}},
  author={Tsimplis, MN and Woolf, DK and Osborn, TJ and Wakelin, S and Wolf, J and Flather, R and Shaw, AGP and Woodworth, P and Challenor, P and Blackman, D and others},
  journal={Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
  volume={363},
  number={1831},
  pages={1329--1358},
  year={2005},
  publisher={The Royal Society}
}



@article{wolf2006waves,
  title={{Waves and climate change in the north-east Atlantic}},
  author={Wolf, Judith and Woolf, David K},
  journal={Geophysical Research Letters},
  volume={33},
  number={6},
  year={2006},
  publisher={Wiley Online Library}
}

@article{woolf2002variability,
  title={{Variability and predictability of the North Atlantic wave climate}},
  author={Woolf, David K and Challenor, PG and Cotton, PD},
  journal={Journal of Geophysical Research: Oceans (1978--2012)},
  volume={107},
  number={C10},
  pages={9--1},
  year={2002},
  publisher={Wiley Online Library}
}



@incollection{hurrell1997decadal,
  title={{Decadal variations in climate associated with the North Atlantic Oscillation}},
  author={Hurrell, James W and Van Loon, Harry},
  booktitle={Climatic Change at High Elevation Sites},
  pages={69--94},
  year={1997},
  publisher={Springer}
}

@article{osborn1999evaluation,
  title={{Evaluation of the North Atlantic Oscillation as simulated by a coupled climate model}},
  author={Osborn, Timothy J and Briffa, Keith R and Tett, Simon FB and Jones, Philip D and Trigo, Ricardo M},
  journal={Climate Dynamics},
  volume={15},
  number={9},
  pages={685--702},
  year={1999},
  publisher={Springer}
}

@article{wanner2001north,
  title={{North Atlantic Oscillation--concepts and studies}},
  author={Wanner, Heinz and Br{\"o}nnimann, Stefan and Casty, Carlo and Gyalistras, Dimitrios and Luterbacher, J{\"u}rg and Schmutz, Christoph and Stephenson, David B and Xoplaki, Eleni},
  journal={Surveys in Geophysics},
  volume={22},
  number={4},
  pages={321--381},
  year={2001},
  publisher={Springer}
}

@article{trigo2006climatology,
  title={{Climatology and interannual variability of storm-tracks in the Euro-Atlantic sector: a comparison between ERA-40 and NCEP/NCAR reanalyses}},
  author={Trigo, Isabel Franco},
  journal={Climate Dynamics},
  volume={26},
  number={2-3},
  pages={127--143},
  year={2006},
  publisher={Springer}
}

@article{trigo2002north,
  title={{The North Atlantic Oscillation influence on Europe: climate impacts and associated physical mechanisms}},
  author={Trigo, Ricardo M and Osborn, Timothy J and Corte-Real, Jo{\~a}o M and others},
  journal={Climate Research},
  volume={20},
  number={1},
  pages={9--17},
  year={2002},
  publisher={INTER-RESEARCH NORDBUNTE 23, D-21385 OLDENDORF LUHE, GERMANY}
}

@article{jones1997extension,
  title={{Extension to the North Atlantic Oscillation using early instrumental pressure observations from Gibraltar and south-west Iceland}},
  author={Jones, PD and Jonsson, T and Wheeler, D},
  journal={International Journal of Climatology},
  volume={17},
  number={13},
  pages={1433--1450},
  year={1997},
  publisher={Wiley Online Library}
}

@article{neill2013wave,
  title={{Wave power variability over the northwest European shelf seas}},
  author={Neill, Simon P and Hashemi, M Reza},
  journal={Applied Energy},
  volume={106},
  pages={31--46},
  year={2013},
  publisher={Elsevier}
}

@article{neill2014inter,
  title={{Inter-annual and inter-seasonal variability of the Orkney wave power resource}},
  author={Neill, Simon P and Lewis, Matt J and Hashemi, M Reza and Slater, Emma and Lawrence, John and Spall, Steven A},
  journal={Applied Energy},
  volume={132},
  pages={339--348},
  year={2014},
  publisher={Elsevier}
}

@article{luterbacher2002reconstruction,
  title={{Reconstruction of sea level pressure fields over the Eastern North Atlantic and Europe back to 1500}},
  author={Luterbacher, J{\"u}rg and Xoplaki, E and Dietrich, D and Rickli, R and Jacobeit, J and Beck, C and Gyalistras, D and Schmutz, C and Wanner, H},
  journal={Climate Dynamics},
  volume={18},
  number={7},
  pages={545--561},
  year={2002},
  publisher={Springer}
}

@article{unden2002hirlam,
  title={{HIRLAM-5 scientific documentation}},
  author={Unden, Per and Rontu, Laura and J{\"a}rvinen, Heikki and Lynch, Peter and Calvo, Javier and Cats, Gerard and Cuxart, Joan and Eerola, Kalle and Fortelius, Carl and Garcia-Moya, Jose Antonio and others},
  year={2002},
  publisher={Citeseer}
}

@article{group1988wam,
  title={{The WAM model-a third generation ocean wave prediction model}},
  author={WAMDI Group, The},
  journal={Journal of Physical Oceanography},
  volume={18},
  number={12},
  pages={1775--1810},
  year={1988}
}

@article{kuttel2010importance,
  title={{The importance of ship log data: reconstructing North Atlantic, European and Mediterranean sea level pressure fields back to 1750}},
  author={K{\"u}ttel, Marcel and Xoplaki, E and Gallego, D and Luterbacher, J and Garcia-Herrera, R and Allan, R and Barriendos, M and Jones, PD and Wheeler, D and Wanner, H},
  journal={Climate Dynamics},
  volume={34},
  number={7-8},
  pages={1115--1128},
  year={2010},
  publisher={Springer}
}



@inproceedings{taylor2009100,
  title={100-year waves, teleconnections and wave climate variability},
  author={Taylor, PH and Barker, VE and Bishop, D and Eatock Taylor, R},
  booktitle={11th International Workshop on Wave Hindcasting and Forecasting, Halifax, Canada},
  year={2009}
}

@book{lamb2002climate,
  title={Climate, History and the Modern World},
  author={Lamb, Hubert H},
  year={2002},
  publisher={Routledge}
}



@article{reistad1998updating,
  title={{Updating, correction and evaluation of a hindcast data base of air pressure, wind and waves for the North Sea, the Norwegian Sea and the Barents Sea}},
  author={Reistad, {\'a}M and Iden, K},
  journal={Res. Rep},
  volume={9},
  year={1998}
}

